Dimensionality Reduction for Sum-of-Distances Metric

We give a dimensionality reduction procedure to approximate the sum of distances of a given set of $n$ points in $R^d$ to any "shape" that lies in a $k$-dimensional subspace. Here, by "shape" we mean any set of points in $R^d$. Our algorithm takes an input in the form of an $n \times d$ matrix $A$, where each row of $A$ denotes a data point, and outputs a subspace $P$ of dimension $O(k^{3}/\epsilon^6)$ such that the projections of each of the $n$ points onto the subspace $P$ and the distances of each of the points to the subspace $P$ are sufficient to obtain an $\epsilon$-approximation to the sum of distances to any arbitrary shape that lies in a $k$-dimensional subspace of $R^d$. These include important problems such as $k$-median, $k$-subspace approximation, and $(j,l)$ subspace clustering with $j \cdot l \leq k$. Dimensionality reduction reduces the data storage requirement to $(n+d)k^{3}/\epsilon^6$ from nnz$(A)$. Here nnz$(A)$ could potentially be as large as $nd$. Our algorithm runs in time nnz$(A)/\epsilon^2 + (n+d)$poly$(k/\epsilon)$, up to logarithmic factors. For dense matrices, where nnz$(A) \approx nd$, we give a faster algorithm, that runs in time $nd + (n+d)$poly$(k/\epsilon)$ up to logarithmic factors. Our dimensionality reduction algorithm can also be used to obtain poly$(k/\epsilon)$ size coresets for $k$-median and $(k,1)$-subspace approximation problems in polynomial time.

==> full-argument.tex <==
\section{Estimating Sum of Distances}
Exact lemma is as follows:
\begin{lemma}
	Let $P$ be the subspace such that for any $k$-dimensional subspace $H$,
	\begin{equation*}
	\sum_i \dist(a_i, P) - \sum_i \dist(a_i, \text{span}(P \cup H)) \le \frac{\epsilon^2}{80}\text{SubApx}_{1,k}(A).
	\end{equation*}
	For such a subspace $P$, we have
$
		\sum_i \dist(\P_{P}a_i,\P_{P \cup H}a_i) \le \epsilon\text{SubApx}_{1,k}(A).
$
\end{lemma}
\begin{proof}
	Let $J \subseteq [n]$ be such that
	$
		\dist(\P_P a_i, \P_{P \cup H}a_i) \le ({\epsilon}/{4})\dist(a_i,P).
	$
	By summing the inequality for all $i \in J$, we get that
	\begin{align*}
		\sum_{i \in J}\dist(\P_Pa_i, \P_{P \cup H}a_i) &\le \frac{\epsilon}{4}\sum_{i \in J}\dist(a_i, P)\\
		&\le \frac{\epsilon}{4}(1+\epsilon)\opt \le \frac{\epsilon}{2}\opt.
	\end{align*}
	Now we consider $i \notin J$. From Pythagorean theorem, we have for all $i$ that
	\begin{equation*}
		\dist(\P_Pa_i, \P_{P \cup H}a_i)^2 = \dist(a_i, P)^2 - \dist(a_i,\text{span}({P \cup H}))^2.
	\end{equation*}
	Additionally, for $i \notin J$
	\begin{equation*}
		\dist(\P_Pa_i, \P_{P \cup H}a_i) \ge \frac{\epsilon}{4}\dist(a_i, P)
	\end{equation*}
	which implies that
	\begin{align*}
		\dist(\P_Pa_i,\P_{P \cup H}a_i) &= \frac{\dist(a_i, P)^2 - \dist(a_i,\text{span}({P \cup H}))^2}{\dist(\P_Pa_i,\P_{P \cup H}a_i)}\\
		&= \frac{(\dist(a_i, P) + \dist(a_i,\text{span}({P \cup H})))(\dist(a_i, P) - \dist(a_i,\text{span}({P \cup H})))}{\dist(\P_Pa_i,\P_{P \cup H}a_i)}\\
		&\le \frac{2\dist(a_i,P)}{\dist(\P_Pa_i, \P_{P \cup H}a_i)}(\dist(a_i,P) - \dist(a_i,\text{span}(P \cup H)))\\
		&\le \frac{8}{\epsilon}(\dist(a_i,P) - \dist(a_i,\text{span}(P \cup H))).
	\end{align*}
	Summing over all $i \notin J$, we obtain
	\begin{equation*}
		\sum_{i \notin J}\dist(\P_Pa_i, \P_{P \cup H}a_i) \le \frac{8}{\epsilon}\sum_{i \notin J}\dist(a_i,P) - \dist(a_i,\text{span}(P \cup H)) \le \frac{\epsilon}{10}\opt.
	\end{equation*}
	Thus $\sum_i \dist(\P_Pa_i, \P_{P \cup H}a_i) \le \epsilon\opt$.
\end{proof}
\begin{theorem}
	If $P$ is a subspace that satisfies
	\begin{equation*}
			\sum_i \dist(a_i, P) - \sum_i \dist(a_i, \text{span}(P \cup H)) \le \frac{\epsilon^2}{80}\opt.
	\end{equation*}
	for any $k$-dimensional subspace $H$, then for any $k$-dimensional shape $S$
	\begin{equation*}
		\sum_{i}\sqrt{\dist(\P_Pa_i, S)^2 + \dist(a_i, P)^2} = (1 \pm 2\epsilon)\sum_i \dist(a_i, S).
	\end{equation*}
\end{theorem}
\begin{proof}
	Let $H$ be the span of $S$. By Pythagorean theorem, for all $i$,
	\begin{equation*}
		\dist(a_i, S) = \sqrt{\dist(a_i, \text{span}(P \cup H))^2 + \dist(\P_{P \cup H}a_i, S)^2}.
	\end{equation*}
	We have
	\begin{align*}
		&|\dist(a_i, S) - \sqrt{\dist(\P_Pa_i, S)^2 + \dist(a_i, P)^2}|\\
		&= |\sqrt{\dist(a_i, \text{span}(P \cup H))^2 + \dist(\P_{P \cup H}a_i, S)^2} - \sqrt{\dist(\P_Pa_i, S)^2 + \dist(a_i, P)^2}|\\
		&\le |\dist(a_i,P) - \dist(a_i,\text{span}(P \cup H))| + |\text{dist}(\P_Pa_i,S) - \text{dist}(\P_{P \cup H}a_i,S)|\\
		&\le |\dist(a_i,P) - \dist(a_i,\text{span}(P \cup H))| + \dist(\P_Pa_i,\P_{P \cup H}a_i).
	\end{align*}
	Summing over all $i$, we obtain
	\begin{equation*}
		\sum_i |\dist(a_i, S) - \sqrt{\dist(\P_Pa_i, S)^2 + \dist(a_i, P)^2}| \le \frac{\epsilon^2}{80}\opt + \epsilon\opt \le 2\epsilon\opt.
	\end{equation*}
	Thus $\sum_i \sqrt{\dist(\P_Pa_i, S)^2 + \dist(a_i, P)^2}$ is a $2\epsilon$ approximation for $\sum_i d(a_i, S)$ for all $k$-dimensional shapes $S$.
\end{proof}

\section{Lopsided Embeddings and Constructions}
\begin{definition}
	A matrix $S$ is a lopsided $\epsilon$-embedding for $(A,B)$ with respect to a constraint set $\mathcal{C}$ and norm $\|\cdot\|$ if
\begin{enumerate}
	\item For all matrices $X$, we have $\|S(AX - B)\| \ge (1 - \epsilon)\|AX-B\|$, and
	\item For $X^* = \argmin_{X \in \mathcal{C}} \|AX-B\|$, the matrix $S$ satisfies $\|S(AX^* - B)\| \le (1+\epsilon)\|AX^* - B\|$.
\end{enumerate}
\end{definition}

We thus have the following theorem
{\color{violet}
\begin{theorem}
	Given a matrix $A \in \R^{n \times d}$ and a parameter $k \le d$, if $\bS \in \R^{m \times d}$ is a random gaussian matrix with number of rows $m = O(k/\epsilon^4 + 1/\epsilon^4\delta^2)$, then with probability $\ge 1 - \delta$ over the choice of $\bS$, 
	\begin{equation*}
		\min_{\text{rank-}k\ X}\|A\bS^TX - A\|_{1,2} \le (1+\epsilon)\min_{\text{rank-}k\ X}\|A(I-X)\|_{1,2}.
	\end{equation*}
\end{theorem}
}
Essentially, a gaussian with $m=O(k/\epsilon^4 + 1/\epsilon^4\delta^2)$ columns works to sketch on the right.

\section{Construction of Well-Conditioned basis using low-distortion embeddings}

Given a matrix $A$, suppose $\bS$ is a random matrix drawn from a distribution such that, with probability $\ge 9/10$, for all vectors $x$
\begin{equation*}
	\alpha\|Ax\|_1 \le \|\bS Ax\|_1 \le \beta\|Ax\|_1.
\end{equation*}
The following theorem gives a construction of well-conditioned basis using a low-distortion subspace embeddings.
\begin{theorem}
	Given a matrix $A \in \R^{n \times d}$, if $\bS$ is a random matrix drawn from a distribution such that with probability $\ge 9/10$,
	\begin{equation*}
		\alpha\|Ax\|_1 \le \|\bS Ax\|_1 \le \beta\|Ax\|_1
	\end{equation*}
	for all vectors $x$. Let $\bS A = QR$ be the $QR$ decomposition of the matrix $A$ where $Q$ is a matrix that has orthonormal columns. Then the matrix $AR^{-1}$ is a {\color{red} $(d\sqrt{r}/\alpha,\beta)$} well-conditioned basis with probability $\ge 9/10$.
\end{theorem}
\begin{proof}
	Assume that for all vectors $x$, we have $\alpha\|Ax\|_1 \le \|\bS Ax\|_1 \le \beta\|Ax\|_1$. Also assume that the matrix $\bS$ has $r$ rows. Now for an arbitrary vector $x$,
	\begin{equation*}
		\|x\|_{\infty} \le \|x\|_2 = \|\bS AR^{-1}x\|_2 \le \|\bS AR^{-1}x\|_1 \le \beta\|AR^{-1}x\|_1.
	\end{equation*}
	Let $e_i$ be $i$th coordinate vector. Then
	\begin{equation*}
		\|AR^{-1}e_i\|_1 \le \frac{1}{\alpha}\|\bS AR^{-1}e_i\|_1 = \frac{\sqrt{r}}{\alpha}\|\bS AR^{-1}e_i\|_2 = \frac{\sqrt{r}}{\alpha}.
	\end{equation*}
	Thus $\sum_{i,j}|(AR^{-1})|_{i,j} = \sum_{i}\|AR^{-1}e_i\| \le d\sqrt{r}/\alpha$.
\end{proof}
\begin{theorem}[Low Distortion Embeddings using Exponential Random Variables, \cite{dw-sketching}]
	Let $\bS$ be an $r \times n$ CountSketch matrix with $r = d \cdot \poly\log(d)$ and $\bD$ be a diagonal matrix with reciprocals of i.i.d standard exponential random variables, then with probability $\ge 9/10$ simultaneously for all vectors $x$, $\alpha\|Ax\|_1 \le \|\bS\bD Ax\|_1 \le \beta\|Ax\|_1$ where $\alpha = O(1/(d\log^{3/2}(d)))$  and $\beta = O(d\log(d))$.
\end{theorem}
Thus we obtain {\color{red} $(d^{5/2}\poly\log(d),d\log(d))$}-well conditioned basis. From Dasgupta et al. we can construct a $1/2$ subspace embedding by sampling $\alpha\beta d = d^{9/2}\poly\log(d)$ rows in expectation by leverage score sampling.


Now, 
\begin{equation*}
	\|\bL A\bS^T X_1(\bL A)^+(\bL A) - \bL A\|_{1,2} \le \|\bL A\bS^T X_1 - \bL A\|_{1,2} \le 10\Delta^*.
\end{equation*}
By above lemma
\begin{equation*}
	\|A\bS^TX_1(\bL A)^+ (\bL A) - A\|_{1,2} \le \left(2 + 20\frac{\sqrt{\text{rank}(X_1(\bL A)^+(\bL A)) + k}}{\alpha}\right)\Delta^* \le (2 + 20\sqrt{2k}/\alpha)\Delta^*.
\end{equation*}

Finally, $\|A(\bL A)^+(\bL A) - A\|_{1,2} \le \left(2 + 20\sqrt{2k}/\alpha\right)\Delta^*$. 

The idea here is that for $\bL$ to be a $\ell_1$ subspace embedding for $A\bS^T$, by lewis weight sampling $\bL$ has only $\tilde{O}(k)$ rows in expectation and only $\tilde{O}(k)$ rows with probability $\ge 9/10$ by a Markov Bound. Thus we get a $(\tilde{O}(\sqrt{k}),\tilde{O}(k))$-bicriteria solution with probability $1/2$ i.e., we obtain a $\tilde{O}(k)$ dimensional subspace $P$ such that 
\begin{equation*}
	\|A\P_P - A\|_{1,2} \le \tilde{O}(\sqrt{k})\Delta^*.
\end{equation*}

By repeating this for $O(\log(1/\delta))$ independent iterations and taking the best subspace we obtain that the above result holds with probability $1 - \delta$. Finding the best subspace can be done by multiplying with a gaussian matrix on the right and finding a constant approximation for all $O(\log(1/\delta))$ subspaces.

\subsection{Constructing Such a matrix \texorpdfstring{$\bL$}{L} by \texorpdfstring{$\ell_1$}{l-1} Leverage Score Sampling}
Given a $n \times d$ matrix $A$, if $\bS$ is a $r \times n$ countsketch matrix, with $r = d \cdot \poly(\log(d))$, and $\bD$ is a diagonal matrix where $\bD_{ii}$ is distributed as reciprocal of a standard exponential random variable, then with probability at least $9/10$, simultaneously for all all vectors $x$,
\begin{equation*}
	\Omega\left(\frac{1}{d\log^{3/2}(d)}\right)\|Ax\|_1 \le \|\bS\bD Ax\|_1 \le O(d \log(d))\|Ax\|_1.
\end{equation*}

If $QW = \bS\bD A$ is the $QW$ decomposition with $Q$ having orthonormal columns and $U = AW^{-1}$, then defining a sampling matrix $\bL$ with probabilities
\begin{equation*}
	q_i = \min(1,O(d^2\log^{5/2}(d))\frac{\|U_{i*}\|_1}{\sum_i \|U_{i*}\|_1})
\end{equation*}
gives a subspace embedding for matrix $A$ satisfying with probability $\ge 9/10$, for all vectors $x$,
\begin{equation*}
	(1/2)\|Ax\|_1 \le \|\bL Ax\|_1 \le (3/2)\|Ax\|_1.
\end{equation*}
Thus, if we can compute the sampling probabilities, we get a subspace of dimension $\Theta(k^{9/2}\log^{5/2}(k))$ that has a cost at most
\begin{equation*}
	\tilde{O}(k^{9/4})\Delta^*.
\end{equation*}
\begin{lemma}
Using a gaussian vector to estimate probabilities, we will have to sample $\tilde{O}(k^{9.5})$ rows. {\color{red} This seems to be too inefficient to implement. It might be better to use more gaussian-columns/or even just use a cauchy matrix with $O(\log(n))$ columns to estimate the probabilities and do with $\nnz{A}\log(n)$ term in the running times than increase the number of rows sampled as for any reasonable $k$ we would've sampled all the rows if we use $k^{9.5}$ algorithm.}
\end{lemma}
\subsection{Sketch of Current algo}
\begin{enumerate}
	\item Given $A$ and a projection matrix $P$, multiply on the right with a gaussian matrix $S$ of $O(k)$ columns.
	\item Find lewis weights of the matrix $A(I-P)G$ and then sample $\tilde{O}(k)$ rows using lewis weights to obtain a sampling matrix $\bL$. Now rowspace of $\bL A(I-P)$ is the potential subspace.
	\item Repeat the above for $O(\log(1/\delta))$ iterations and return the best subspace.
\end{enumerate}
\section{Residual Sampling}{\label{sec:Proof of Residual Sampling}}
%Suppose we are given a projection matrix $X$ such that
%\begin{equation*}
%	\|A(I - X)\|_{1,2} \le K \Delta^*.
%\end{equation*}
%Define $z'_{i} = \|A_{i*}(I-X)\|_2$ and define $z_i = \min(1, rz_i'/\sum_i z_i')$ for some $r$. If $\bS$ is a sampling matrix formed with the probability vector $z$, we want to show that if $Y$ spans the rows of $X$ and $\bS A$, then with good probability, $Y$ spans a good rank-$k$ subspace to project rows of $A$ on to.
%
%Let $r$ be the number of rows in $\bS A$. Order the rows of $\bS A$ arbitrarily. For $l \in [r]$, let $H_l$ denote the space spanned by rows of $X$ along with first $l$ rows of $\bS A$. The $l$th sample is in phase $j$ if there exists a rank $k$ projection matrix $X_j$ such that
%\begin{enumerate}
%	\item  $G := \text{rspace}(X_j) \cap H_l$ has a dimension at least $j$, and
%	\item $\|A(I-X_j)\|_{1,2} \le (1 + \delta)^j\Delta^*$ for $\delta = \epsilon/2k$.
%\end{enumerate}
%
%Thus $X^*$ satisfies the requirements for $X_0$. Let $Y_l$ denote the rank-$k$ projection matrix by rotating the subspace rspace($X_j$) about $G$ so as to contain the smallest nonzero principal angle between $H_l$ and $\text{rspace}(X_j)$. Thus dimension of the subspace $\text{rspace}(Y_l) \cap H_l$ is $= j' > j$ and $Y_l$ \emph{could} potentially be $X_j'$ for some $j' > j$.
%
%If $\|A(I-Y_l)\|_{1,2} \le (1+\delta)\|A(I-X_j)\|_{1,2}$, then we are in phase $j' > j$ and there is nothing to do. So, assume that $\|A(I-Y_l)\|_{1,2} > (1+\delta)\|A(I-X_j)\|$. 



Given a projection matrix $\hat{X}$ such that $\|A(I - \hat{X})\| \le K\Delta^*$, let $p_i$ for $i \in [n]$ be such that $p_i \ge \alpha\|A_{i*}(I-\hat{X})\|_{2}/\|A(I-\hat{X})\|_{1,2}$ for some $1 \le \alpha > 0$ and $\sum_{i}p_i = 1$. If $S$ is a set of i.i.d samples from the distribution over $[n]$ defined by the probability vector $p$, then for $|S| \ge \ldots$, subspace spanned by $\hat{X} \cup A_S$ spans a $k$-dimensional subspace that is a $1+\epsilon$ approximation for sum-of-distances subspace approximation.

Let the sampled indices be divided into $k+1$ phases indexed by $0,\ldots,k$. The sampling process is in phase $j$ if the current subset $S$ is such that there exists a $k$-dimensional subspace $F_j$ satisfying
\begin{enumerate}
	\item  $\text{dim}(F_j \cap \text{span}(A_{S} \cup \hat{X})) \ge j$, and
	\item $\|A(I - \P_{F_j})\|_{1,2} \le (1+\delta)^j\Delta^*$.
\end{enumerate}
Thus once the sampling is in phase $j$, it remains in phase $j'$ for some $j' \ge j$ in subsequent steps. Let $S_j$ denote $S$ when the sampling is in phase $j$ for the very first time. Define $G_j = F_j \cap \text{span}(A_{S_j} \cup \hat{X})$. Note that $G_j$ is at least a $j$ dimensional subspace. We want to upperbound the expected number of steps the sampling can be in phase $j$. Define $F_j^o = G_j^{\perp} \cap F_j$ and $V^o = G_j^\perp \cap \text{span}(A_S \cup \hat{X})$. Let $l$ be the line in subspace $F_j^o$ that makes the smallest angle with the subspace $V^o$. Let $l^o$ be the line in $V^o$ that makes this angle with $l$. Let $\hat{F}^o$ be the rotation of $F_j^o$ to include the line $l^o$ and let $\hat{F} = \text{span}(\hat{F}^o \cup G_j)$. Note that $\text{dim}(\hat{F} \cap \text{span}(A_{S} \cup \hat{X})) > \text{dim}(G_j)$. Thus $\hat{F}$ could potentially be $F_{j'}$ for some $j' > j$. 

Given the current sample $S$, and the subspaces $\hat{F}^o$ and $F_j^o$, we call a step \emph{good} if we sample $A_{i*}$ in the step that satisfies
\begin{enumerate}
	\item The sample $S$ in phase $k$ or 
	\item $\|A_{i*}(I-\P_{G_j})(I-\P_{\hat{F}^o})\|_2 > (1+\delta/2)\|A_{i*}(I-\P_{G_j})(I-\P_{F_j^o})\|_2$.
\end{enumerate}
Note that the subspaces $\hat{F}^o$ and $F_j^o$ are orthogonal to the subspace $G$ and therefore we have $\P_G\P_{\hat{F}^o} = \P_G\P_{F_j^o} = 0$. We also have from the definitions of the subspaces that $\P_G + \P_{\hat{F}^o} = \P_{\hat{F}}$ and $\P_{G} + \P_{F_j^o} = \P_{F_j}$. Thus the second condition can be equivalently written as
\begin{equation*}
	\|A_{i*}(I - \P_{\hat{F}})\|_2 > (1+\delta/2)\|A_{i*}(I-\P_{F_j})\|_2.
\end{equation*}
Theorem 9 from \cite{deshpande2007sampling} shows that there can only be at most $O(1/\delta\log(K/\delta))$ good steps in a phase. Let $W \subseteq [n]$ be the subset of indices that are good with respect to the sample $S$. We claim the following: If $\|A(I-\P_{\hat{F}})\|_{1,2} > (1+\delta)\|A(I-\P_{F_j})\|_{1,2}$, then
\begin{equation*}
	\|A_{W*}(I-\P_{\hat{X}})\|_{1,2} \ge \frac{\delta}{4K}\|A(I-\P_{\hat{X}})\|_{1,2}.
\end{equation*}
We prove this by showing a contradiction by assuming that the above doesn't hold. For any index $i$,
\begin{align*}
	\|A_{i*}(I-\P_{\hat{F}})\|_2 &\le \|A_{i*}(I-\P_{A_S \cup \hat{X}})(I-\P_{\hat{F}})\|_2 + \|A_{i*}\P_{A_S \cup \hat{X}}(I-\P_{\hat{F}})\|_2\\
	&\le \|A_{i*}(I-\P_{A_S \cup \hat{X}})\|_2 + \|A_{i*}\P_{A_S \cup \hat{X}}(I-\P_{\hat{F}})\|_2\\
	&\le \|A_{i*}(I-\P_{A_S \cup \hat{X}})\|_2 + \|A_{i*}\P_{A_S \cup \hat{X}}(I-\P_{F_j})\|_2\\
	&\text{Since $\hat{F}$ is obtained by rotating $F_j$ about $G_j$ to be closer to $A_S \cup \hat{X}$}\\
	&\le 2\|A_{i*}(I-\P_{A_S \cup \hat{X}})\|_2 + \|A_{i*}(I-\P_{F_j})\|_2\\
	&\le 2\|A_{i*}(I-\P_{\hat{X}})\|_2 + \|A_{i*}(I-\P_{F_j})\|_2.
\end{align*}
 As we already have that for \emph{not good} indices $i$ that $\|A_{i*}(I-\P_{\hat{F}})\|_2 \le (1+\delta/2)\|A_{i*}(I-\P_{F_j})\|_2$, we obtain that for all $i$
 \begin{equation*}
 	\|A_{i*}(I-\P_{\hat{F}})\|_2 \le (1+\delta/2)\|A_{i*}(I-\P_{F_j})\|_2 + 2[i \in W]\|A_{i*}(I-\P_{\hat{X}})\|_2
 \end{equation*}
 which implies that
 \begin{align*}
 	\|A(I-\P_{\hat{F}})\|_{1,2} &\le (1+\delta/2)\|A(I-\P_{F_j})\|_{1,2} + 2\|A_{W*}(I-\P_{\hat{X}})\|_{1,2}\\
 	&\le (1+\delta/2)\|A(I-\P_{F_j})\|_{1,2} + 2\frac{\delta}{4K}\|A(I-\P_{\hat{X}})\|_{1,2}\\
 	&\le (1+\delta/2)\|A(I-\P_{F_j})\|_{1,2} + (\delta/2)\Delta^*\\
 	&\le (1+\delta)\|A(I - \P_{F_j})\|_{1,2} \le (1+\delta)^{j+1}\Delta^*,
 \end{align*}
 which is a contradiction to our assumption that the sampling process $S$ is still in phase $j$. Thus $\sum_{i \in W}p_i \ge \alpha\sum_{i \in W}\|A_{i*}(I - \P_{\hat{X}})\|_2/\|A(I-\P_{\hat{X}})\|_{1,2} \ge (\alpha\delta/4K)$. Thus every step is \emph{independently} a \emph{good} step with probability at least $(\alpha\delta/4K)$. Thus it is easy to see that with probability $\ge 1 - \delta$, the algorithm is in phase $k$ in $N = O(K/\alpha \cdot k^3\epsilon^{-2}\log(k \cdot K/\epsilon))$ steps. Thus sampling each $i \in [n]$ independently with probability $\min(1, Np_i)$ also satisfies the same bounds.
 
 \if 0
 \section{Lewis Weights Sampling to construct \texorpdfstring{$\ell_1$}{l-1} subspace embeddings}
Let $A \in \R^{n \times d}$ be a given matrix and $a_1,\ldots,a_n$ be the vectors corresponding to $n$ rows of the matrix $A$. The $\ell_1$ lewis weights $w_1,\ldots,w_n$ are defined as the positive real numbers that satisfy
\begin{equation*}
	a_i^T(A^TW^{-1}A)^{-1}a_i = w_i^2
\end{equation*}
where $W = \text{diag}(w_1,\ldots,w_n)$. It can be shown that lewis weights exist and they are unique.

	\begin{algorithm}[htbp]
	\DontPrintSemicolon
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwData{Start}{start}
    \SetKwData{End}{end}
		\caption{\textsc{LewisIterate}}
		\label{alg:lewis-iterate}
			\Input{$A\in\R^{n\times d}$, $w \in \R^{n}$}
			\Output{$\hat{w} \in \R^n$}
			$\tilde{\tau} \in \R^n \gets $ 2-approximate statistical leverage scores of the matrix $(\text{diag}(w_1,\ldots,w_n))^{-1/2}A$\;
			$\hat{w}_i \gets (w_i\tilde{\tau}_i)^{1/2}$ for all $i \in [n]$\;
			\Return{$\hat{w}$}
	\end{algorithm}
	
	\begin{algorithm}[htbp]
	\DontPrintSemicolon
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwData{Start}{start}
    \SetKwData{End}{end}
		\caption{\textsc{ApproxLewisWeights}}
		\label{alg:approx-lewis}
			\Input{$A\in\R^{n\times d}$}
			\Output{$w \in \R^n$}
			$w \gets 1^n$\;
			$T \gets \log_2\log_2(n)$\;
			\For{$i  = 1,\ldots,T$}{
				$w \gets \textsc{LewisIterate}(A,w)$\;
			}
			\Return{$w$}
	\end{algorithm}
	\begin{theorem}
		Given a matrix $A \in \R^{n \times d}$, the Algorithm~\ref{alg:approx-lewis} returns a vector $w \in \R^{n}$ such that $(1/4)w_i \le \overline{w}_i \le 4w_i$ for all $i$ where $\overline{w} \in \R^n$ denotes lewis weights of the matrix $A$.
	\end{theorem}
	Sampling using the $4$-approximate lewis weights returned by the Algorithm, we can sample $O(d\log(d))$ rows and obtain a sampling-and-scaling matrix $\bS$ such that with probability $O(1)$ probability $(1/2)\|Ax\|_1 \le \|\bS Ax\|_1 \le 2\|Ax\|_1$ for all $x$ and $\E_{\bS}[\|\bS M\|_{1,2}] = \|M\|_{1,2}$ for any matrix $M$.
\fi
